When Do LLMs Help With Node Classification? A Comprehensive Analysis

Node classification is a fundamental task in graph analysis, with broad applications across various fields. Recent breakthroughs in Large Language Models (LLMs) have enabled LLM-based approaches for this task. Although many studies demonstrate the impressive performance of LLM-based methods, the lack of clear design guidelines may hinder their practical application. In this work, we aim to establish such guidelines through a fair and systematic comparison of these algorithms. As a first step, we developed LLMNodeBed, a comprehensive codebase and testbed for node classification using LLMs. It includes 10 homophilic datasets, 4 heterophilic datasets, 8 LLM-based algorithms, 8 classic baselines, and 3 learning paradigms. Subsequently, we conducted extensive experiments, training and evaluating over 2,700 models, to determine the key settings (e.g., learning paradigms and homophily) and components (e.g., model size and prompt) that affect performance. Our findings uncover 8 insights, e.g., (1) LLM-based methods can significantly outperform traditional methods in a semi-supervised setting, while the advantage is marginal in a supervised setting; (2) Graph Foundation Models can beat open-source LLMs but still fall short of strong LLMs like GPT-4o in a zero-shot setting. We hope that the release of LLMNodeBed, along with our insights, will facilitate reproducible research and inspire future studies in this field. Codes and datasets are released at \href{https://llmnodebed.github.io/}{\texttt{https://llmnodebed.github.io/}}.

==> tables/old/mainexp.tex <==
\begin{table*}[!t]
    \centering
    \caption{\textbf{Overall Performance Comparison under Fully-supervised Setting.} The \colorbox{blue!20}{\textbf{best}} and \colorbox{blue!10}{runner-up} results are highlighted.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|cccccccccc}
      \toprule
      \rowcolor{COLOR_MEAN} & & \multicolumn{4}{c}{\textbf{Academic}} & \textbf{Web Link} & \multicolumn{2}{c}{\textbf{Social}} & \multicolumn{3}{c}{\textbf{E-Commerce}} \\
      \rowcolor{COLOR_MEAN} \multicolumn{2}{c}{\multirow{-2}{*}{\textbf{Accuracy (\%)}}}   & Cora & Citeseer & Pubmed & arXiv & WikiCS & Instagram & Reddit & Books-History & Ele-Photo & Ele-Computers \\ \midrule

      \multicolumn{2}{c|}{GCN$_{\text{ShallowEmb}}$} & 87.41$_{\pm \text{2.08}}$ & 75.74$_{\pm \text{1.20}}$ & 89.01$_{\pm \text{0.59}}$ & 71.39$_{\pm \text{0.28}}$ & 83.67$_{\pm \text{0.63}}$ & 63.94$_{\pm \text{0.61}}$ & 65.07$_{\pm \text{0.38}}$ & 76.94$_{\pm \text{0.26}}$ & 73.34$_{\pm \text{1.34}}$ & 77.16$_{\pm \text{3.80}}$ \\ 
      \multicolumn{2}{c|}{SAGE$_{\text{ShallowEmb}}$} & 87.44$_{\pm \text{1.74}}$ & 74.96$_{\pm \text{1.20}}$ & 90.47$_{\pm \text{0.25}}$ & 71.21$_{\pm \text{0.18}}$ & 84.86$_{\pm \text{0.91}}$ & 64.14$_{\pm \text{0.47}}$ & 61.52$_{\pm \text{0.60}}$ & 79.40$_{\pm \text{0.45}}$ & 84.59$_{\pm \text{0.32}}$ & 87.77$_{\pm \text{0.34}}$ \\

      \multicolumn{2}{c|}{GAT$_{\text{ShallowEmb}}$} & 86.68$_{\pm \text{1.12}}$ & 73.73$_{\pm \text{0.94}}$ & 88.25$_{\pm \text{0.47}}$ & 71.57$_{\pm \text{0.25}}$ & 83.94$_{\pm \text{0.61}}$ & 64.93$_{\pm \text{0.75}}$ & 64.16$_{\pm \text{1.05}}$ & 80.61$_{\pm \text{0.49}}$ & 84.84$_{\pm \text{0.69}}$ & 88.32$_{\pm \text{0.24}}$ \\ \midrule
      
      \multicolumn{2}{c|}{RoBERTa-355M} & 83.17$_{\pm \text{0.84}}$ & 75.90$_{\pm \text{1.69}}$ & \cellcolor{blue!20} \textbf{94.84$_{\pm \text{0.06}}$} & 74.12$_{\pm \text{0.12}}$ & \cellcolor{blue!20}\textbf{87.47$_{\pm \text{0.83}}$} & 63.75$_{\pm \text{1.13}}$ & 60.61$_{\pm \text{0.24}}$ & 
      \cellcolor{blue!20} \textbf{86.65$_{\pm \text{0.38}}$} & 79.45$_{\pm \text{0.37}}$ & 75.76$_{\pm \text{0.30}}$ \\ \midrule
      
      \multirow{2}{*}{\textbf{Encoder}} & $\text{GCN}_{\text{LLMEmb}}$ & 
      \cellcolor{blue!20} \textbf{88.15$_{\pm \text{1.79}}$} & \cellcolor{blue!10} 76.45$_{\pm \text{1.19}}$ & 88.38$_{\pm \text{0.68}}$ & 74.39$_{\pm \text{0.31}}$ & 84.78$_{\pm \text{0.86}}$ & 68.27$_{\pm \text{0.45}}$ & 70.65$_{\pm \text{0.75}}$ & 84.23$_{\pm \text{0.20}}$ & 86.07$_{\pm \text{0.20}}$ & 89.52$_{\pm \text{0.31}}$ \\ 
      & ENGINE & 87.00$_{\pm \text{1.60}}$ & 75.82$_{\pm \text{1.52}}$ & 90.08$_{\pm \text{0.16}}$ & 74.69$_{\pm \text{0.36}}$ & 85.44$_{\pm \text{0.53}}$ & \cellcolor{blue!10} 68.87$_{\pm \text{0.25}}$ & \cellcolor{blue!20} \textbf{71.21$_{\pm \text{0.77}}$} & 84.09$_{\pm \text{0.09}}$ & 86.98$_{\pm \text{0.06}}$ & 89.05$_{\pm \text{0.13}}$ \\  \midrule
      \textbf{Reasoner} & TAPE &  \cellcolor{blue!10} 88.05$_{\pm \text{1.76}}$ & 76.45$_{\pm \text{1.60}}$ & 93.00$_{\pm \text{0.13}}$ & \cellcolor{blue!10} 74.96$_{\pm \text{0.14}}$ & \cellcolor{blue!10} 87.11$_{\pm \text{0.66}}$ & 68.11$_{\pm \text{0.54}}$ & 66.22$_{\pm \text{0.83}}$ & \cellcolor{blue!10} 85.95$_{\pm \text{0.59}}$ & \cellcolor{blue!20} \textbf{87.72$_{\pm \text{0.28}}$} & \cellcolor{blue!20} \textbf{90.46$_{\pm \text{0.18}}$} \\  \midrule
      \multirow{3}{*}{\textbf{Predictor}} & $\text{LLM}_{\text{IT}}$ & 71.93$_{\pm \text{1.47}}$ & 58.94$_{\pm \text{3.26}}$ & \cellcolor{blue!10} 93.80$_{\pm \text{0.13}}$ & \cellcolor{blue!20} \textbf{76.08} & 78.66$_{\pm \text{1.14}}$ & 43.77$_{\pm \text{3.21}}$ & 58.30$_{\pm \text{0.48}}$ & 84.80$_{\pm \text{0.13}}$ & 78.27$_{\pm \text{0.54}}$ & 74.51$_{\pm \text{0.53}}$ \\ 
      & GraphGPT \\ 
      & LLaGA & 87.55$_{\pm \text{1.15}}$ & \cellcolor{blue!20} \textbf{76.73$_{\pm \text{1.70}}$} & 90.28$_{\pm \text{0.91}}$ & 74.49$_{\pm \text{0.23}}$ & 84.03$_{\pm \text{1.10}}$ & \cellcolor{blue!20} \textbf{69.16$_{\pm \text{0.72}}$} & \cellcolor{blue!10} 71.06$_{\pm \text{0.38}}$ & 85.56$_{\pm \text{0.30}}$ & \cellcolor{blue!10} 87.62$_{\pm \text{0.30}}$ & \cellcolor{blue!10} 90.41$_{\pm \text{0.12}}$ \\ \bottomrule
    \end{tabular}
    }

    \vspace*{5pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|cccccccccc}
      \toprule
      \rowcolor{COLOR_MEAN} \multicolumn{2}{c}{\textbf{Macro-F1 (\%)}}   & Cora & Citeseer & Pubmed & arXiv & WikiCS & Instagram & Reddit & Books-History & Ele-Photo & Ele-Computers \\ \midrule
      \multicolumn{2}{c|}{GCN$_{\text{ShallowEmb}}$} & 86.54$_{\pm \text{1.44}}$ & 71.52$_{\pm \text{1.71}}$ & 88.54$_{\pm \text{0.60}}$ & 50.28$_{\pm \text{0.84}}$ & 82.11$_{\pm \text{0.61}}$ & 54.91$_{\pm \text{0.48}}$ & 65.00$_{\pm \text{0.42}}$ & 34.39$_{\pm \text{1.26}}$ & 66.04$_{\pm \text{2.85}}$ & 64.60$_{\pm \text{4.99}}$ \\ 

      \multicolumn{2}{c|}{SAGE$_{\text{ShallowEmb}}$} & 86.37$_{\pm \text{1.26}}$ & 71.87$_{\pm \text{1.34}}$ & 90.16$_{\pm \text{0.27}}$ & 49.73$_{\pm \text{0.49}}$ & 82.78$_{\pm \text{1.53}}$ & 51.37$_{\pm \text{1.67}}$ & 61.39$_{\pm \text{0.54}}$ & 38.29$_{\pm \text{2.54}}$ & 80.37$_{\pm \text{0.34}}$ & 82.93$_{\pm \text{0.49}}$ \\ 
      \multicolumn{2}{c|}{GAT$_{\text{ShallowEmb}}$} & 85.64$_{\pm \text{0.87}}$ & 69.27$_{\pm \text{2.15}}$ & 87.70$_{\pm \text{0.48}}$ & 49.71$_{\pm \text{0.23}}$ & 82.14$_{\pm \text{1.04}}$ & 50.26$_{\pm \text{3.16}}$ & 64.11$_{\pm \text{1.06}}$ & 42.85$_{\pm \text{1.62}}$ & 80.82$_{\pm \text{0.89}}$ & 84.74$_{\pm \text{0.79}}$ \\ \midrule
      
      \multicolumn{2}{c|}{RoBERTa-355M} & 81.38$_{\pm \text{1.17}}$ & 72.31$_{\pm \text{1.45}}$ & \cellcolor{blue!20} \textbf{94.33$_{\pm \text{0.14}}$} & 57.25$_{\pm \text{0.53}}$ & \cellcolor{blue!20} \textbf{86.10$_{\pm \text{1.11}}$} & 59.10$_{\pm \text{1.38}}$ & 60.16$_{\pm \text{0.94}}$ & \cellcolor{blue!20} \textbf{57.24$_{\pm \text{1.27}}$} & 72.89$_{\pm \text{0.50}}$ & 70.64$_{\pm \text{0.58}}$ \\ \midrule
      \multirow{2}{*}{\textbf{Encoder}} & $\text{GCN}_{\text{LLMEmb}}$ & \cellcolor{blue!20} \textbf{87.23$_{\pm \text{1.34}}$} & 
      \cellcolor{blue!10} 72.71$_{\pm \text{0.86}}$ & 87.76$_{\pm \text{0.76}}$ & 55.22$_{\pm \text{0.46}}$ & 82.78$_{\pm \text{1.68}}$ & \cellcolor{blue!20} \textbf{60.38$_{\pm \text{0.53}}$} & \cellcolor{blue!10} 70.64$_{\pm \text{0.75}}$ & 48.18$_{\pm \text{2.29}}$ & 80.51$_{\pm \text{0.65}}$ & 85.10$_{\pm \text{1.00}}$ \\ 
      & ENGINE & 85.72$_{\pm \text{1.58}}$ & 71.22$_{\pm \text{2.17}}$ & 89.63$_{\pm \text{0.14}}$ & 56.32$_{\pm \text{0.60}}$ & 83.80$_{\pm \text{1.06}}$ & \cellcolor{blue!10} 60.02$_{\pm \text{1.26}}$ & \cellcolor{blue!20} \textbf{71.17$_{\pm \text{0.75}}$} & 48.24$_{\pm \text{2.64}}$ & 82.77$_{\pm \text{0.28}}$ & 84.15$_{\pm \text{0.84}}$ \\  \midrule
      \textbf{Reasoner} & TAPE & \cellcolor{blue!10} 87.21$_{\pm \text{1.60}}$ & \cellcolor{blue!20} \textbf{73.33$_{\pm \text{1.57}}$} & 92.39$_{\pm \text{0.02}}$ & \cellcolor{blue!10} 57.79$_{\pm \text{0.49}}$ & \cellcolor{blue!10} 86.03$_{\pm \text{1.14}}$ & 58.31$_{\pm \text{1.15}}$ & 65.91$_{\pm \text{0.71}}$ & 54.07$_{\pm \text{2.01}}$ & \cellcolor{blue!10} 83.41$_{\pm \text{0.42}}$ & \cellcolor{blue!10} 86.78$_{\pm \text{0.53}}$ \\  \midrule
      \multirow{3}{*}{\textbf{Predictor}} & $\text{LLM}_{\text{IT}}$ & 66.93$_{\pm \text{4.54}}$ \\ 
      % & 63.30$_{\pm \text{3.87}}$ & 32.54$_{\pm \text{1.39}}$ & \cellcolor{blue!10} 93.07$_{\pm \text{0.09}}$ & 57.48 & 76.67$_{\pm \text{0.50}}$ & 41.72$_{\pm \text{4.56}}$ & 56.65$_{\pm \text{0.85}}$ & 49.13$_{\pm \text{1.19}}$ & 68.74$_{\pm \text{2.54}}$ & 55.25$_{\pm \text{2.83}}$ \\ 
      & GraphGPT \\ 
      & LLaGA & 84.97$_{\pm \text{3.97}}$ & 72.59$_{\pm \text{1.70}}$ & 90.00$_{\pm \text{0.80}}$ & \cellcolor{blue!20} \textbf{58.08$_{\pm \text{0.29}}$} & 82.37$_{\pm \text{1.73}}$ & 57.96$_{\pm \text{2.40}}$ & 62.14$_{\pm \text{15.59}}$ & \cellcolor{blue!10} 54.89$_{\pm \text{2.29}}$ & \cellcolor{blue!20} \textbf{83.56$_{\pm \text{0.40}}$} & \cellcolor{blue!20} \textbf{86.97$_{\pm \text{0.34}}$} \\ \bottomrule
    \end{tabular}
    }
   % \label{tab:main_exp}
\end{table*}

==> tables/old/mainexp_semi.tex <==
\begin{table*}[!t]
    \centering
    \caption{\textbf{Overall Performance Comparison under Semi-supervised Setting.} The \colorbox{blue!20}{\textbf{best}} and \colorbox{blue!10}{runner-up} results are highlighted.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccccccccc}
      \toprule
      \rowcolor{COLOR_MEAN} & & \multicolumn{3}{c}{\textbf{Academic}} & \textbf{Web Link} & \multicolumn{2}{c}{\textbf{Social}} & \multicolumn{3}{c}{\textbf{E-Commerce}} \\
     \rowcolor{COLOR_MEAN} \multicolumn{2}{c}{\multirow{-2}{*}{\textbf{Accuracy (\%)}}}   & Cora & Citeseer & Pubmed & WikiCS & Instagram & Reddit & Books-History & Ele-Photo & Ele-Computers \\ \midrule
         \multicolumn{2}{c|}{GCN$_{\text{ShallowEmb}}$} & 82.30$_{\pm \text{0.19}}$ & 70.55$_{\pm \text{0.32}}$ & \cellcolor{blue!20} \textbf{78.94$_{\pm \text{0.27}}$} & 79.86$_{\pm \text{0.19}}$ & 63.50$_{\pm \text{0.11}}$ & 61.44$_{\pm \text{0.38}}$ & 68.79$_{\pm \text{0.46}}$ & 69.25$_{\pm \text{0.81}}$ & 71.44$_{\pm \text{1.19}}$ \\ 
         \multicolumn{2}{c|}{SAGE$_{\text{ShallowEmb}}$} & 82.27$_{\pm \text{0.37}}$ & 69.56$_{\pm \text{0.43}}$ & 77.88$_{\pm \text{0.44}}$ & 79.67$_{\pm \text{0.25}}$ & 63.57$_{\pm \text{0.10}}$ & 56.65$_{\pm \text{0.33}}$ & 72.01$_{\pm \text{0.33}}$& 78.50$_{\pm \text{0.15}}$ & 81.43$_{\pm \text{0.27}}$ \\ 
          \multicolumn{2}{c|}{GAT$_{\text{ShallowEmb}}$} & 81.30$_{\pm \text{0.67}}$ & 69.94$_{\pm \text{0.74}}$ & 78.49$_{\pm \text{0.70}}$ & 79.99$_{\pm \text{0.65}}$ & 63.56$_{\pm \text{0.04}}$ & 60.60$_{\pm \text{1.17}}$ & 74.35$_{\pm \text{0.35}}$ & 80.40$_{\pm \text{0.45}}$ & 83.39$_{\pm \text{0.22}}$ \\ 
         \midrule 
         \multicolumn{2}{c|}{RoBERTa-355M} & 72.24$_{\pm \text{1.14}}$ & 66.68$_{\pm \text{2.03}}$ & 42.32$_{\pm \text{1.56}}$ & 76.81$_{\pm \text{1.04}}$ & 63.52$_{\pm \text{0.44}}$ & 59.27$_{\pm \text{0.34}}$ & \cellcolor{blue!10} 84.62$_{\pm \text{0.16}}$ & 74.79$_{\pm \text{1.13}}$ & 72.31$_{\pm \text{0.37}}$ \\ \midrule
         
        \multirow{2}{*}{\textbf{Encoder}} 
       & $\text{GCN}_{\text{LLMEmb}}$ & 83.33$_{\pm \text{0.75}}$ & 71.39$_{\pm \text{0.90}}$ & \cellcolor{blue!10} 78.71$_{\pm \text{0.45}}$ & \cellcolor{blue!10} 80.94$_{\pm \text{0.16}}$ & \cellcolor{blue!20} \textbf{67.49$_{\pm \text{0.43}}$} & 68.65$_{\pm \text{0.75}}$ &  83.03$_{\pm \text{0.34}}$ & \cellcolor{blue!10} 84.84$_{\pm \text{0.47}}$ & \cellcolor{blue!10} 88.22$_{\pm \text{0.16}}$ \\ 
       & ENGINE & \cellcolor{blue!20} \textbf{84.22$_{\pm \text{0.46}}$} & \cellcolor{blue!20} \textbf{72.14$_{\pm \text{0.74}}$}
        & 77.84$_{\pm \text{0.27}}$ & 80.94$_{\pm \text{0.19}}$ & \cellcolor{blue!10} 67.14$_{\pm \text{0.46}}$ & \cellcolor{blue!10} 69.67$_{\pm \text{0.16}}$ & 82.89$_{\pm \text{0.14}}$ & 84.33$_{\pm \text{0.57}}$ & 86.42$_{\pm \text{0.23}}$ \\  \midrule
        
       \textbf{Reasoner} & TAPE &  \cellcolor{blue!10} 84.04$_{\pm \text{0.24}}$ & \cellcolor{blue!10} 71.87$_{\pm \text{0.35}}$ & 78.61$_{\pm \text{1.23}}$ & \cellcolor{blue!20} \textbf{81.94$_{\pm \text{0.16}}$} & 66.07$_{\pm \text{0.10}}$ & 62.43$_{\pm \text{0.47}}$ & \cellcolor{blue!20} \textbf{84.92$_{\pm \text{0.26}}$} & \cellcolor{blue!20} \textbf{86.46$_{\pm \text{0.12}}$} & \cellcolor{blue!20} \textbf{89.52$_{\pm \text{0.04}}$} \\  \midrule
       
      \multirow{3}{*}{\textbf{Predictor}} & $\text{LLM}_{\text{IT}}$  &  67.00$_{\pm \text{0.16}}$ & 53.70$_{\pm \text{0.94}}$ & 68.99$_{\pm \text{8.14}}$ & 74.32$_{\pm \text{1.06}}$ & 41.19$_{\pm \text{0.84}}$ & 54.09$_{\pm \text{1.02}}$ & 80.92$_{\pm \text{1.38}}$ & 71.28$_{\pm \text{1.81}}$ & 66.99$_{\pm \text{2.02}}$ \\ 
       & GraphGPT \\ 
       & LLaGA & 78.94$_{\pm \text{1.14}}$ & 62.61$_{\pm \text{3.63}}$ & 65.91$_{\pm \text{2.09}}$ & 76.47$_{\pm \text{2.20}}$ & 65.84$_{\pm \text{0.72}}$ &  \cellcolor{blue!20} \textbf{70.10$_{\pm \text{0.38}}$} & 83.47$_{\pm \text{0.45}}$ & 84.44$_{\pm \text{0.90}}$ & 87.82$_{\pm \text{0.53}}$ \\
       \bottomrule
    \end{tabular}
    }

   \vspace*{5pt}
   \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccccccccc}
      \toprule
     \rowcolor{COLOR_MEAN} \multicolumn{2}{c}{\textbf{Macro-F1 (\%)}}   & Cora & Citeseer & Pubmed & WikiCS & Instagram & Reddit & Books-History & Ele-Photo & Ele-Computers \\ \midrule
         \multicolumn{2}{c|}{GCN$_{\text{ShallowEmb}}$} & 80.76$_{\pm \text{0.30}}$ & 66.00$_{\pm \text{0.17}}$ & \cellcolor{blue!20} \textbf{79.00$_{\pm \text{0.30}}$} & 77.87$_{\pm \text{0.18}}$ & 52.44$_{\pm \text{1.02}}$ & 61.15$_{\pm \text{0.56}}$ & 22.18$_{\pm \text{1.12}}$ & 62.65$_{\pm \text{1.46}}$ & 61.33$_{\pm \text{2.55}}$ \\ 
          \multicolumn{2}{c|}{SAGE$_{\text{ShallowEmb}}$} & 80.88$_{\pm \text{0.47}}$ & 65.06$_{\pm \text{0.32}}$ & 77.88$_{\pm \text{0.41}}$ & 77.02$_{\pm \text{0.59}}$ & 50.74$_{\pm \text{0.26}}$ & 56.39$_{\pm \text{0.44}}$ & 24.37$_{\pm \text{0.72}}$ & 74.17$_{\pm \text{0.32}}$ & 71.67$_{\pm \text{0.61}}$ \\ 
          \multicolumn{2}{c|}{GAT$_{\text{ShallowEmb}}$} & 79.65$_{\pm \text{1.03}}$ & 64.82$_{\pm \text{1.20}}$ & 78.43$_{\pm \text{0.73}}$ & 77.57$_{\pm \text{1.01}}$ & 40.19$_{\pm \text{1.56}}$ & 60.37$_{\pm \text{1.22}}$ & 28.93$_{\pm \text{3.65}}$ & 75.89$_{\pm \text{0.60}}$ & 77.06$_{\pm \text{2.98}}$\\ 
         \midrule 
          \multicolumn{2}{c|}{RoBERTa-355M} & 70.41$_{\pm \text{0.83}}$ & 63.36$_{\pm \text{1.75}}$ & 40.82$_{\pm \text{2.05}}$ & 73.98$_{\pm \text{1.72}}$ & \cellcolor{blue!10} 57.43$_{\pm \text{0.42}}$ & 59.23$_{\pm \text{0.36}}$ & \cellcolor{blue!20} \textbf{51.34$_{\pm \text{0.95}}$} & 67.92$_{\pm \text{0.49}}$ & 63.38$_{\pm \text{2.17}}$ \\ \midrule
          
        \multirow{2}{*}{\textbf{Encoder}}  
       & $\text{GCN}_{\text{LLMEmb}}$ & 81.19$_{\pm \text{0.59}}$ & \cellcolor{blue!20} \cellcolor{blue!20} \textbf{67.17$_{\pm \text{0.73}}$} & 78.39$_{\pm \text{0.36}}$ & 78.58$_{\pm \text{0.51}}$ & \cellcolor{blue!20} \textbf{58.97$_{\pm \text{0.85}}$} & \cellcolor{blue!10} 68.46$_{\pm \text{0.91}}$ & 39.64$_{\pm \text{0.85}}$ & \cellcolor{blue!10} 79.87$_{\pm \text{0.57}}$ & 77.36$_{\pm \text{0.70}}$\\ 
       & ENGINE & \cellcolor{blue!20} \textbf{82.52$_{\pm \text{0.45}}$} & \cellcolor{blue!10} \textbf{67.15$_{\pm \text{0.15}}$} & 77.53$_{\pm \text{0.34}}$ & \cellcolor{blue!10} 78.89$_{\pm \text{0.38}}$ & 57.25$_{\pm \text{2.50}}$ & \cellcolor{blue!20} \textbf{69.56$_{\pm \text{0.21}}$} & 34.04$_{\pm \text{1.10}}$ & 78.55$_{\pm \text{1.12}}$ & 75.86$_{\pm \text{0.60}}$  \\  \midrule
       
       \textbf{Reasoner} & TAPE & \cellcolor{blue!10} 81.89$_{\pm \text{0.31}}$ & 66.80$_{\pm \text{0.33}}$ & \cellcolor{blue!10} 78.46$_{\pm \text{1.13}}$ & \cellcolor{blue!20} \textbf{80.03$_{\pm \text{0.23}}$} & 50.01$_{\pm \text{1.60}}$ & 61.23$_{\pm \text{0.69}}$ & \cellcolor{blue!10} 47.12$_{\pm \text{3.26}}$ & \cellcolor{blue!20} \textbf{82.31$_{\pm \text{0.19}}$} & \cellcolor{blue!20} \textbf{84.90$_{\pm \text{1.14}}$} \\  \midrule
       
      \multirow{3}{*}{\textbf{Predictor}} & $\text{LLM}_{\text{IT}}$ & 56.35$_{\pm \text{0.22}}$ \\
      % & 30.77$_{\pm \text{7.05}}$ & 28.04$_{\pm \text{0.92}}$ & 0.31$_{\pm \text{0.16}}$ & 51.22$_{\pm \text{3.55}}$ & 37.07$_{\pm \text{1.63}}$ & 23.79$_{\pm \text{7.61}}$ &  33.32$_{\pm \text{5.38}}$ & 44.16$_{\pm \text{6.19}}$ & 34.54$_{\pm \text{5.63}}$ \\ 
       & GraphGPT \\ 
       & LLaGA  & 71.14$_{\pm \text{4.47}}$ & 52.53$_{\pm \text{3.59}}$ & 45.12$_{\pm \text{7.63}}$ & 70.48$_{\pm \text{2.94}}$ & 50.12$_{\pm \text{10.45}}$ & 54.67$_{\pm \text{11.24}}$ & 39.70$_{\pm \text{2.44}}$ & 79.32$_{\pm \text{2.42}}$ & \cellcolor{blue!10} 78.01$_{\pm \text{1.36}}$ \\ \bottomrule
    \end{tabular}
    }
   %  \label{tab:mainexp_semi}
\end{table*}
